ARWalker: A Virtual Walking Companion Application

Extended Reality (XR) technologies, including Augmented Reality (AR), have attracted significant attention over the past few years and have been utilized in several fields, including education, healthcare, and manufacturing. In this paper, we aim to explore the use of AR in the field of biomechanics and human movement through the development of ARWalker, which is an AR application that features virtual walking companions (avatars). Research participants walk in close synchrony with the virtual companions, whose gait exhibits properties found in the gait of young and healthy adults. As a result, research participants can train their gait to the gait of the avatar, thus regaining the healthy properties of their gait and reducing the risk of falls. ARWalker can especially help older adults and individuals with diseases, who exhibit pathological gait thus being more prone to falls. We implement a prototype of ARWalker and evaluate its systems performance while running on a Microsoft Hololens 2 headset.

==> sections/Material_and_Method.tex <==
\section{Materials And Methods}
\label{sec:material} 
TBD - Brief description of patient trials~\cite{hololens1}

\subsection{Apparatus}
TBD - Brief description of motion capture system and the specifications such as number of cameras, camera quality etc.

\subsubsection{Virtual Elements}
To combine the virtual elements with the real world, we used Microsoft Hololens 2 with eye tracking and hand tracking enabled. The Hololens 2 has a display resolution of 2048 x 1080 pixels per eye. 

The virtual elements are mainly comprised of a UI and an Avatar. The user can select an avatar from a diverse group of avatars. This was designed to aid the user through complexity matching \cite{complexity-matching} and the proteus effect \cite{proteus:effect}. For example, there has been credible evidence that avatar appearance and body type influence the users \cite{vr:body1, vr:body2, vr:skincolor1}.  To further extend the sense of realism to generate the illusory effect of body ownership \cite{vr:bodyRealism}, we used realistic humanoid avatars coupled with high-quality, motion-captured walk animations. 

\subsection{Approaches}
To design our application, we use the Unity game engine %(V 2021.1.14f1) 
with the Mixed Reality Toolkit %(V 2.7.2) 
(MRTK) and OpenXR. %(V 1.2.8). 
The Unity game engine provides a design environment and a set of functions such as physics and animation controls. The MRTK enables quick prototyping, UX design, and XR-specific common set of functions such as hand and environment tracking. OpenXR provides abstraction between user experience and different XR platforms such as Hololens and Oculus. This allows our application to run on multiple platforms with a few changes. %During our design iterations, 
We designed and developed different approaches, which we describe below. 

\subsubsection{Baseline (Self-Paced) Version }

This is the baseline version of our experiment. The goal of this phase is to provide a reference for the Mixed Reality (MR) gait conditions. The measurements in this phase are based on a self-paced natural gait of the participant without any device or other additional materials. The data were collected while participants walked on a track field for a few minutes. % add the number of iterations and the minutes once we have trial details.

\subsubsection{Naive AR Based Metronome}

A metronome describes an assistive device that is used for gait rehabilitation in older adults and other clinical populations. These metronomes are based on the optimal movement variability hypothesis~\cite{Optimal-movement-variability}, which provides a baseline to characterize systems that are less adaptable such as abnormal motor development or unhealthy states. According to this hypothesis, the gait of healthy individuals have certain statistical properties (a ''pink-noise'' (or 1/f noise, representing fractal processes that are both stable and flexible \cite{NoiseTypes}) frequency distribution of steps) over time. Due to aging or diseases, individuals may lose these properties (pathological gait), but their gait can be trained to restore these properties. Overall, gait metronomes incorporate properties of the optimal movement variability hypothesis in their operation to help individuals with pathological gait restore the properties of healthy gait. For example, an auditory metronome may feature a beat that follows a ``pink-noise'' distribution, so that individuals can synchronize their gait to the beat of the metronome~\cite{Likens2021}.

\begin{figure}[!t]
 \centering
 \includegraphics[width=0.7\columnwidth]{pictures/NoAvatar.png}
 \caption{The design of our naive AR based gait metronome running on Microsoft Hololens 2.}
 \label{Figure:naivedesign}
\end{figure}

%\includegraphics{pictures/NoAvatar.png} \newline
%\centering
%\textbf{Figure 1:} The design of our AR-based gait metronome running on Microsoft Hololens 2 headsets.\newline

In Figure~\ref{Figure:naivedesign}, we present the design of our naive AR based metronome. In our metronome, we provide visual stimuli in the form of a bar that moves vertically. When the bar reaches the highest point, participants are instructed to touch the ground with their feet as they are taking a step forward. The movement of the vertical bar is based on different frequency distributions. The first available distribution is ''pink noise'' (representing healthy gait), the second is ''brown noise'' (representing processes that are stable but unable to flexibly modify their activity when rapid changes are required \cite{NoiseTypes}), and the third one is a random distribution.

\subsubsection{Avatar Based Metronome}

On a high level, our metronome application work as follows. At the start of the application, it allows users to choose an avatar from a diverse pool of avatars. In Figures~\ref{Figure:avatarfemale} and~\ref{Figure:avatarmale}, we present our avatar-based metronome with a male and female avatar from our avatar pool. After that, the selected avatar will spawn in front of the user. %Then, the user also can select a gait pattern that simulates different walking patterns. 
When the user starts walking, the selected avatar will walk in front of the user staying in the user's field of view. Our hypothesis is that through context matching the user will restore the complexity of their own gait by synchronizing their gait to the gait of the avatar. %The realistic nature of the mixed reality will enhance the rehabilitation process through the illusory effect of body ownership. 
During our design iterations, we designed and developed three different versions of our avatar based metronome, which we describe below.

\begin{figure}[!t]
%\vspace{-0.5cm}
    %\captionsetup[subfigure]{aboveskip=-0.1pt,belowskip=-0.1pt}
	\centering
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\includegraphics[width=1\columnwidth]{pictures/SUF.pdf}
		%\vspace{-0.5cm}
		\caption{A female avatar.} \hfill
		\label{Figure:avatarfemale}
	\end{subfigure} 
	\hfill
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\includegraphics[width=1\columnwidth]{pictures/SUM.pdf}
		%\vspace{-0.5cm}
		\caption{A male avatar.}  \hfill
		\label{Figure:avatarmale}
	\end{subfigure}
	\vspace{-0.5cm}
	\caption{Our avatar-based gait metronome.}
	\vspace{-0.2cm}
\end{figure}

% \begin{figure}[!t]
%  \centering
%  \includegraphics[width=0.7\columnwidth]{pictures/SU1.jpg}
%  \caption{The avatar-based gait metronome running on Microsoft Hololens 2 with a female avatar.}
%  \label{Figure1:avatarfemale}
% \end{figure}

% \begin{figure}[!t]
%  \centering
%  \includegraphics[width=0.7\columnwidth]{pictures/SU2.jpg}
%  \caption{The avatar-based gait metronome running on Microsoft Hololens 2 with a male avatar.}
%  \label{Figure:avatarmale}
% \end{figure}

\begin{figure}[!t]
%\vspace{-0.5cm}
    %\captionsetup[subfigure]{aboveskip=-0.1pt,belowskip=-0.1pt}
	\centering
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\includegraphics[width=1\columnwidth]{pictures/Waypoint.pdf}
		%\vspace{-0.5cm}
		\caption{A male avatar walking in front of the user's field of view.} \hfill
		\label{Figure:avatarfemalewalking}
	\end{subfigure} 
	\hfill
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\includegraphics[width=1\columnwidth]{pictures/Follow.pdf}
		%\vspace{-0.5cm}
		\caption{A humanoid avatar walking in front of the user's field of view.}  \hfill
		\label{Figure:avatarmalewalking}
	\end{subfigure}
	\vspace{-0.5cm}
	\caption{Different avatars walking in front of the user's field of view.}
	\vspace{-0.2cm}
\end{figure}

% \begin{figure}[!t]
%  \centering
%  \includegraphics[width=0.7\columnwidth]{pictures/Waypoint.jpg}
%  \caption{Avatar-based gait metronome waypoint version.}
%  \label{Figure:avatarmale}
% \end{figure}

% \begin{figure}[!t]
%  \centering
%  \includegraphics[width=0.7\columnwidth]{pictures/FollowMe.jpg}
%  \caption{Avatar-based gait metronome followme version.}
%  \label{Figure:avatarmale}
% \end{figure}

\noindent \textbf{Scene understanding:} Our first version utilizes MRTK's scene understanding observer and Unity NavMesh. MRTK's scene understanding observer provides a powerful computer vision library that can be used to recognize environmental objects, such as walls, floors, meshes, and quads. The Unity NavMesh component allows to bake a map of walkable and unwalkable areas. Using scene understanding, we recognize the environment and extract the quads, which are the physics engine-friendly 2D surfaces that occupy the 3D world, such as the surface area of the floor or a table. We than bake a NavMesh on top of the quads of the floor by defining walkable and unwalkable areas. This process is dynamic and can adapt to a changing environment to a certain extent. Once we have a NavMesh, an Artificial Intelligence (AI) agent called NavMesh agent can utilize this data for intelligent navigation. This allows our avatar to roam the environment in a realistic manner by avoiding obstacles and reacting to a changing environment. %Figures 2 and 3, present the design of the Hololens 2 scene understanding version along with avatars.  

\noindent \textbf{Waypoint:} In our second version, we removed the scene understanding and NavMesh system to save processing power and memory. Instead of using an AI agent for intelligent navigation, we allow the user to define a navigation path by adding waypoints. This approach introduces a calibration process to the system. In the first run, the user has to define a path for the avatar by placing waypoints. After that user can save this path locally for future use. We create a separate UI for this calibration process. After defining the path, the avatar will move from waypoint to waypoint on a preset path and the user can follow the avatar for gait rehabilitation. %Figure 4, presents the design of the waypoint version alone with an avatar. 

\noindent \textbf{Head tracking:} Compared to the other two solutions, this is simple and easier to implement. We use a solver handler function in MRTK to track the head position of a user. By using head movements, the avatar turns in the same way as the user's head. We also implemented a singleton instance that calculates the user's speed, distance, and rotations. Whenever the user starts to move, this signals the animation to start and transit the avatar from idle to a walking animation. This approach allows the user to navigate in any environment in a light-weight manner in terms of the occupied resources (CPU and memory usage) of the headset.

%with the least amount of resources, overhe and time. %Figure 5, presents the design of the head tracking version alone with an avatar.  
